Ranking Catamorphisms and Unranking Anamorphisms on Hereditarily Finite Datatypes

Using specializations of unfold and fold on a generic tree data type we derive unranking and ranking functions providing natural number encodings for various Hereditarily Finite datatypes. In this context, we interpret unranking operations as instances of a generic anamorphism and ranking operations as instances of the corresponding catamorphism. Starting with Ackerman's Encoding from Hereditarily Finite Sets to Natural Numbers we define pairings and tuple encodings that provide building blocks for a theory of Hereditarily Finite Functions. The more difficult problem of ranking and unranking Hereditarily Finite Permutations is then tackled using Lehmer codes and factoradics. The self-contained source code of the paper, as generated from a literate Haskell program, is available at \url{http://logic.csci.unt.edu/tarau/research/2008/fFUN.zip}. Keywords: ranking/unranking, pairing/tupling functions, Ackermann encoding, hereditarily finite sets, hereditarily finite functions, permutations and factoradics, computational mathematics, Haskell data representations

==> TOOLS/spheader.tex <==
\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{subfig}
\usepackage{url}
\usepackage{verbatim} 
\usepackage{listings}
\lstloadlanguages{Prolog}
\lstnewenvironment{code}
    {\lstset{}%
      \csname lst@SetFirstLabel\endcsname}
    {\csname lst@SaveFirstLabel\endcsname}
    \lstset{
      basicstyle=\small\ttfamily,
      flexiblecolumns=false,
      basewidth={0.5em,0.45em},
      literate={+}{{$+$}}1 {*}{{$*$}}1 {=}{{$=$}}1
               {>}{{$>$}}1 {<}{{$<$}}1
               {<-}{{$\leftarrow$}}2
               {|}{{$\mid$}}1               
    }
\newtheorem{prop}{Proposition}
\newtheorem{df}{Definition}

\def \bscale1 {1.00}
\def \bscale {0.20}
\def \hscale {0.20}

% \FIG{Label}{Title}{PNG}
\newcommand{\FIG}[3]{
\begin{figure}[htbp]
\centering
\scalebox{\bscale1}{\includegraphics*[bb=0pt 0pt 800pt 800pt]{./figs/#3.png}}
\caption{#2}
\label{#1}
\end{figure}
}

% \HFIGS{Label}{Title}{Title1}{Title2}{PNG1}{PNG2}
\newcommand{\HFIGS}[6]{
\begin{figure}[htbp]
  \centering
  \subfloat[#3]{
    {\scalebox{\hscale}{\includegraphics*[bb=0pt 0pt 800pt 800pt]
    {./figs/#5.png}}}} 
  \subfloat[#4]{
    {\scalebox{\hscale}{\includegraphics*[bb=0pt 0pt 800pt 800pt]
    {./figs/#6.png}}}}
  \caption{#2}
  \label{#1}
\end{figure}
}

% \VFIGS{Label}{Title}{Title1}{Title2}{PNG1}{PNG2}
\newcommand{\VFIGS}[6]{
\begin{figure}[htbp]
  \begin{center}
    {\scalebox{\bscale}{\includegraphics*[bb=0pt 0pt 800pt 800pt]{./figs/#5.png}}}
    {\scalebox{\bscale}{\includegraphics*[bb=0pt 0pt 800pt 800pt]{./figs/#6.png}}}
  \caption{#2: {\em #3} and {\em #4}}
  \label{#1}
  \end{center}
\end{figure}
}

